The Luttinger-Kohn theory for multiband Hamiltonians: A revision of ellipticity requirements

Modern applications require a robust and theoretically solid tool for the realistic modeling of electronic states in low dimensional nanostructures. The $k \cdot p$ theory has fruitfully served this role for the long time since its establishment. During the last three decades several problems have been detected in connection with the application of the $k \cdot p$ approach to such nanostructures. These problems are closely related to the violation of the ellipticity conditions for the underlying model, the fact that has been largely overlooked in the literature. We derive ellipticity conditions for $6 \times 6$, $8\times 8$ and $14 \times 14$ Hamiltonians obtained by the application of Luttinger-Kohn theory to the bulk zinc blende (ZB) crystals, and demonstrate that the corresponding models are non-elliptic for many common crystalline materials. With the aim to obtain the admissible (in terms of ellipticity) parameters, we further develop and justify a parameter rescaling procedure for $8\times 8$ Hamiltonians. This allows us to calculate the admissible parameter sets for GaAs, AlAs, InAs, GaP, AlP, InP, GaSb, AlSb, InSb, GaN, AlN, InN. The newly obtained parameters are then optimized in terms of the bandstructure fit by changing the value of the inversion asymmetry parameter $B$ that is proved to be essential for ellipticity of $8\times 8$ Hamiltonian. The consecutive analysis, performed here for all mentioned $k \cdot p$ Hamiltonians, indicates the connection between the lack of ellipticity and perturbative terms describing the influence of out-of-basis bands on the structure of the Hamiltonian. This enables us to quantify the limits of models' applicability material-wise and to suggest a possible unification of two different $14 \times 14$ models, analysed in this work.

==> figures/fig2/plots.tex <==
%% LaTeX2e file `plots.tex'
%% generated by the `filecontents' environment
%% from source `sample' on 2018/08/03.
%%
  \csvloop
  {
   file={data.csv},
   no head, column count=4, column names reset,
   column names={1=\one, 2=\two, 3=\three, 4=\four},
%   command= \one  \two  \three  \four,
   command={\addplot[mark=*] coordinates {(\one,\two)}},
   late after line={{;} }
  }


==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	//
Acknowledgements	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section*{Acknowledgements}$/;"	s
Conclusions	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section*{Conclusions}$/;"	s
DLKnonel	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{DLKnonel}$/;"	l
Eight-band Hamiltonians	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section{Eight-band Hamiltonians}\\label{sec8x8}$/;"	s
Ellipticity analysis for $8 times 8$ ZB Hamiltonian with inversion-asymmetry present	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\subsection{Ellipticity analysis for $8 \\times 8$ ZB Hamiltonian with inversion-asymmetry pres/;"	u	section:Eight-band Hamiltonians
Ellipticity analysis in the absence of inversion asymmetry	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\subsection{Ellipticity analysis in the absence of inversion asymmetry}%conduction-valence band/;"	u	section:Eight-band Hamiltonians
Ellipticity of $14 times 14$ band models	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section{Ellipticity of $14 \\times 14$ band models}$/;"	s
Introduction	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section{Introduction}$/;"	s
Overview of Luttinger-Kohn bandstructure theory	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section{Overview of Luttinger-Kohn bandstructure theory }$/;"	s
QF	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{QF}$/;"	l
SEBC	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\label{SEBC}$/;"	l
SchrodEqs	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{SchrodEqs}$/;"	l
Six-bands Hamiltonian analysis	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section{Six-bands Hamiltonian analysis}\\label{sec6x6}$/;"	s
article_codes	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^Naturally, the results presented here remains valid\\footnote{\\label{article_codes} All computa/;"	l
condKane_gamma_B_zero	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{condKane_gamma_B_zero}$/;"	l
eigZB14P	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eigZB14P}$/;"	l
eig_LK	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eig_LK}$/;"	l
eiginKaneN	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eiginKaneN}$/;"	l
eq:4x4constrB	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq:4x4constrB}$/;"	l
eq:A  _exp	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq:A'_exp}$/;"	l
eq:Kane_Ep_adj	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq:Kane_Ep_adj}$/;"	l
eq:Kane_eig_a	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\label{eq:Kane_eig_a}$/;"	l
eq:Kane_range_delta	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq:Kane_range_delta}$/;"	l
eq:ZBK_delta05_sel	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq:ZBK_delta05_sel}$/;"	l
eq:eigQFKP4x4	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq:eigQFKP4x4}$/;"	l
eq:el_constrZBKane_nzB	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq:el_constrZBKane_nzB}$/;"	l
eq:inneqQFKP4x4	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq:inneqQFKP4x4}$/;"	l
eqConvLLm	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eqConvLLm}$/;"	l
eqConvLLpp	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eqConvLLpp}$/;"	l
eqHKane4	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eqHKane4}$/;"	l
eqZBBPHam	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^  \\label{eqZBBPHam}$/;"	l
eq_PO	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eq_PO}$/;"	l
eqineig	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{eqineig}$/;"	l
fig:DLK	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^  \\label{fig:DLK}$/;"	l
fig:ZBK_rescB_34_bs_comp:GaAs	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\label{fig:ZBK_rescB_34_bs_comp:GaAs}$/;"	l
fig:ZBK_rescB_80_bs_comp:GaAs	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\label{fig:ZBK_rescB_80_bs_comp:GaAs}$/;"	l
fig:ZBK_resc_bs_comp	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\label{fig:ZBK_resc_bs_comp}$/;"	l
fig:ZBK_resc_bs_comp:GaN	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\label{fig:ZBK_resc_bs_comp:GaN}$/;"	l
pdo	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\begin{equation}\\label{pdo}$/;"	l
sec6x6	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section{Six-bands Hamiltonian analysis}\\label{sec6x6}$/;"	l
sec8x8	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^\\section{Eight-band Hamiltonians}\\label{sec8x8}$/;"	l
tabMPZBL14x14resc	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\label{tabMPZBL14x14resc} $/;"	l
tabMPZBL6x6	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\label{tabMPZBL6x6} \\tabcolsep=0.4em $/;"	l
tabMPZBL8x8	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\label{tabMPZBL8x8} $/;"	l
tabMPZBL8x8optB	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\caption{Results of bandstructure error minimization procedures based on the adjustment of $B$/;"	l
tabMPZBL8x8optBd	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\caption{Results of direct bandstructure error minimization procedures based on the adjustment/;"	l
tabMPZBL8x8resc	/home/d314/doc/doc_win/statti/Band_structures/Ellipticity/2submission/prb/ellipt.tex	/^	\\label{tabMPZBL8x8resc} $/;"	l

